Assessing the Answerability of Queries in Retrieval-Augmented Code Generation

Thanks to unprecedented language understanding and generation capabilities of large language model (LLM), Retrieval-augmented Code Generation (RaCG) has recently been widely utilized among software developers. While this has increased productivity, there are still frequent instances of incorrect codes being provided. In particular, there are cases where plausible yet incorrect codes are generated for queries from users that cannot be answered with the given queries and API descriptions. This study proposes a task for evaluating answerability, which assesses whether valid answers can be generated based on users' queries and retrieved APIs in RaCG. Additionally, we build a benchmark dataset called Retrieval-augmented Code Generability Evaluation (RaCGEval) to evaluate the performance of models performing this task. Experimental results show that this task remains at a very challenging level, with baseline models exhibiting a low performance of 46.7%. Furthermore, this study discusses methods that could significantly improve performance.

==> tables/ICL+RAG_prompt_for_patent.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[t!]
\centering
\caption{Example prompt for answerability verification. If the query is answerable, then the language model further generates a response from a prompt with instructions to continue.}
\label{tab:ICL-prompt}
\begin{tabular}{|l|}
\hline
\begin{tabular}[c]{@{}l@{}}\# Profile\\ - Role: AnswerabilityVerificationGPT, evaluating whether provided documents can support answering\\  the user's questions effectively.\\ \\ \# Input\\ - Question: User's specific question(s).\\ - Candidate Documents: Documents potentially useful for answering the questions.\\ \\ \# Skill\\ 1. Analyzing questions to understand the required information.\\ 2. Assessing documents to determine their ability to support clear and accurate answers.\\ \\ \# Rules\\ 1. Maintain character.\\ 2. Provide final verdict only as "{[}Answerable{]}" or "{[}Unanswerable{]}".\\ 3. Do not evaluate demonstration, only assess question(s) and documents.\\ 4. Adhere strictly to output format.\\ \\ \# Judgment Criteria\\ 1. Document length should not influence evaluation.\\ 2. Strive for objectivity.\\ 3. "{[}Answerable{]}" if documents support clear, accurate, and engaging answers, "{[}Unanswerable{]}" otherwise.\\ \\ \# Workflow\\ 1. Understand user questions.\\ 2. Evaluate documents for answer support.\\ 3. Provide final judgment.\\ \\ \# Reminder\\ Always remember the role settings.\\ \\ Question: \{\{query\}\}\\ \\ Candidate Documents\\ \{\{apis\}\}\\ \\ Judgment: \\ \\ (If [Answerable]) Answer the user question with using given APIs:
\end{tabular} \\ \hline
\end{tabular}
\end{table*}

==> tables/codegen_pass_w_cov.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\caption{Code generation performance with various answerability verifier and code generator. The quality of the answerability verification model is measured with pass@k (k=1,10)}
\label{tab:codegen_pass_w_cov}
\begin{tabular}{|cccc|ccc|}
\hline
\multicolumn{4}{|c|}{Answerability verification} &
  \multicolumn{3}{c|}{Code generation} \\ \hline
\multicolumn{2}{|c|}{Model} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}f1\\ (\%)\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}coverage (c)\\ (\%)\end{tabular}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{Model}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}  $\mathbb{E}_{c}[pass@1]$ \\\ (\%)\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\mathbb{E}_{c}[pass@10]$\\ (\%)\end{tabular}} \\ \cline{1-2}
Backbone &
  \multicolumn{1}{c|}{Method} &
   &
   &
  \multicolumn{1}{c|}{} &
   &
   \\ \hline
\multicolumn{2}{|c|}{no verifier} &
  N/A &
  100 &
  \multicolumn{1}{c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}codellama-\\ 7b-\\ instruct\end{tabular}}} &
  18.8 &
  37.5 \\ \cline{1-4} \cline{6-7} 
gpt-3.5-turbo &
  \multicolumn{1}{c|}{CoT + ICL-3w2s} &
  50.7 &
  64.9 &
  \multicolumn{1}{c|}{} &
  19.1 &
  36.6 \\ \cline{1-4} \cline{6-7} 
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}codellama-\\ 7b-instruct\end{tabular}} &
  \multicolumn{1}{c|}{CoT + ICL-3w2s} &
  33.5 &
  (0,100{]} &
  \multicolumn{1}{c|}{} &
  20.7 &
  39.0 \\
 &
  \multicolumn{1}{c|}{QLoRA + NegAug} &
  54.5 &
  (0,100{]} &
  \multicolumn{1}{c|}{} &
  25.1 &
  45.4 \\ \cline{1-4} \cline{6-7} 
\multicolumn{2}{|c|}{human verification} &
  100.0 &
  36.5 &
  \multicolumn{1}{c|}{} &
  26.6 &
  47.3 \\ \hline
\multicolumn{2}{|c|}{no verifier} &
  N/A &
  100.0 &
  \multicolumn{1}{c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}llama-3-\\ 8b-\\ instruct\end{tabular}}} &
  17.4 &
  34.6 \\ \cline{1-4} \cline{6-7} 
gpt-3.5-turbo &
  \multicolumn{1}{c|}{CoT + ICL-3w2s} &
  50.7 &
  64.9 &
  \multicolumn{1}{c|}{} &
  18.6 &
  36.6 \\ \cline{1-4} \cline{6-7} 
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}llama-3-\\ 8b-instruct\end{tabular}} &
  \multicolumn{1}{c|}{CoT + ICL-3w2s} &
  52.4 &
  (0,100{]} &
  \multicolumn{1}{c|}{} &
  20.7 &
  38.1 \\
 &
  \multicolumn{1}{c|}{QLoRA + NegAug} &
  64.0 &
  (0,100{]} &
  \multicolumn{1}{c|}{} &
  23.0 &
  40.5 \\ \cline{1-4} \cline{6-7} 
\multicolumn{2}{|c|}{human verification} &
  100.0 &
  36.5 &
  \multicolumn{1}{c|}{} &
  25.4 &
  43.2 \\ \hline
\end{tabular}
\end{table*}

==> tables/codegen_pass_w_cov_0528.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\caption{Code generation performance with various answerability verifier and code generator. The quality of the answerability verification model is measured with pass@k (k=1,10)}
\label{tab:codegen_pass_w_cov_0528}
\begin{tabular}{|cc|cc|cc|}
\hline
\multicolumn{2}{|c|}{Model} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}accuracy\\ (\%)\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}coverage(c)\\ (\%)\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\mathbb{E}_{c}[pass@1]$\\ (\%)\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\mathbb{E}_{c}[pass@10]$\\ (\%)\end{tabular}} \\ \cline{1-2}
Backbone                                                                        & Method         &       &           &      &      \\ \hline
\multicolumn{2}{|c|}{no verifier}                                                                & N/A   & 100       & 16.6 & 34.2 \\ \hline
gpt-3.5-turbo                                                                   & CoT + ICL-3w2s & 34.4  & 47.1      & 19.1 & 40.2 \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}llama-3-\\ 8b-instruct\end{tabular}} & CoT + ICL-3w2s & 51.8  & (0,100{]} & 22.6 & 42.7 \\
                                                                                & QLoRA + NegAug & 54.6  & (0,100{]} & 23.9 & 43.3 \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}gemma-1.1-\\ 7b-it\end{tabular}}     & CoT + ICL-3w2s & 47.2  & (0,100{]} & 20.0 & 36.6 \\
                                                                                & QLoRA + NegAug & 56.3  & (0,100{]} & 22.0 & 40.9 \\ \hline
\multicolumn{2}{|c|}{human verification}                                                         & 100.0 & 36.5      & 24.1 & 45.4 \\ \hline
\end{tabular}
\end{table*}

==> tables/codegen_pass_w_cov_0530.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\caption{Code generation performance with various answerability verifier. The quality of the answerability verification model is measured with pass@k (k=1,10)}
\label{tab:codegen_pass_w_cov_0528}
\begin{tabular}{|ccl|cc|cc|}
\hline
\multicolumn{3}{|c|}{Model} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}accuracy\\ (\%)\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}coverage(c)\\ (\%)\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}$\mathbb{E}_{c}[pass@1]$\\ (\%)\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}$\mathbb{E}_{c}[pass@10]$\\ (\%)\end{tabular}} \\ \cline{1-3}
\multicolumn{1}{|c|}{\multirow{2}{*}{Backbone}}                                                       & \multicolumn{2}{c|}{Method} &       &               &      &      \\ \cline{2-3}
\multicolumn{1}{|c|}{}                                                                                & Fine-tune           & Inference &       &               &      &      \\ \hline
\multicolumn{3}{|c|}{no verifier}                                                                                                   & N/A   & 100           & 16.6 & 34.2 \\ \hline
\multicolumn{1}{|c|}{gpt-3.5-turbo}                                                                   & X               & ICL-3w2s  & 34.4  & 47.1          & 19.1 & 40.2 \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}llama-3-\\ 8b-instruct\end{tabular}}} & X               & ICL-3w2s  & 51.8  & (0,100{]} & 22.6 & 42.7 \\
\multicolumn{1}{|c|}{}                                                                                & QLoRA + NegAug  & ICL-3w2s  & 54.6  & (0,100{]} & 23.8 & 43.2 \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{gemma-1.1-}\\ \textbf{7b-it}\end{tabular}}}     & X               & ICL-3w2s  & 47.2  & (0,100{]} & 20.0 & 36.6 \\
\multicolumn{1}{|c|}{}                                                                                & \textbf{QLoRA + NegAug}  & \textbf{ICL-3w2s}  & \textbf{56.3}  & \textbf{(0,100{]}} & \textbf{23.6} & \textbf{42.5} \\ \hline
\multicolumn{3}{|c|}{human verification}                                                                                            & 100.0 & 36.5          & 24.1 & 45.4 \\ \hline
\end{tabular}
\end{table*}

==> tables/codegen_pass_w_cov_0531.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\caption{The performance of coding RAG pipeline in Figure~\ref{fig:RAGdiag_with_AV}. The generated code quality is measured with pass@k (k=1,10)}
\label{tab:codegen_pass_w_cov_0528}
\begin{tabular}{|ccl|cc|cc|}
\hline
\multicolumn{3}{|c|}{Model} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}accuracy\\ (\%)\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}coverage(c)\\ (\%)\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}$\mathbb{E}_{c}[pass@1]$\\ (\%)\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}$\mathbb{E}_{c}[pass@10]$\\ (\%)\end{tabular}} \\ \cline{1-3}
\multicolumn{1}{|c|}{\multirow{2}{*}{Backbone}}                                                       & \multicolumn{2}{c|}{Method} &       &               &      &      \\ \cline{2-3}
\multicolumn{1}{|c|}{}                                                                                & Fine-tune           & Inference &       &               &      &      \\ \hline
\multicolumn{3}{|c|}{no verifier}                                                                                                   & N/A   & 100           & 16.6 & 34.2 \\ \hline
\multicolumn{1}{|c|}{gpt-3.5-turbo}                                                                   & X               & ICL-3w2s  & 42.9  & 47.1          & 19.1 & 40.2 \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}llama-3-\\ 8b-instruct\end{tabular}}} & X               & Zero-shot  & 48.9  & (0,100{]} & 17.8 & 34.4 \\
\multicolumn{1}{|c|}{}                                                                                & QLoRA + NegAug  & ICL-3w2s  & 54.0  & (0,100{]} & \textbf{23.8} & \textbf{43.2} \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}gemma-1.1-\\ 7b-it\end{tabular}}}     & X               & Zero-shot  & 49.7  & (0,100{]} & 20.4 & 38.8 \\
\multicolumn{1}{|c|}{}                                                                                & QLoRA + NegAug  & ICL-3w2s  & \textbf{59.3}  & (0,100{]} & 23.6 & 42.5 \\ \hline
\multicolumn{3}{|c|}{human verification}                                                                                            & 100.0 & 36.5          & 24.1 & 45.4 \\ \hline
\end{tabular}
\end{table*}

==> tables/query_reformulate_prompt.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[b!]
\caption{examples of 4-shot query reformulation prompts constructed using various interrogatives.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|}
\hline
\begin{tabular}[c]{@{}l@{}}\# Profile\\ You are a query reformulater to make the given query look natural.\\ \\ \# Inputs\\ \\ \#\# Query\\ I'd like to calculate element-wise average between a, b and c. Next, multiply numsets rowwise \\ Basically out{[}i{]} = a{[}i{]} * b{[}i{]}, where a{[}i{]}.shape is (2,) and b{[}i{]} then is a scalar. What's the trick?\\ \\ \#\# Response\\ How can I calculate the element-wise average between a, b, and c? Also, how can I multiply the \\ elements of numsets row-wise using the formula out{[}i{]} = a{[}i{]} * b{[}i{]}, where a{[}i{]} has a shape of \\ (2,) and b{[}i{]} is a scalar?\\ \\ \#\# Query\\ Take samples from these DataPipes based on their weights with random seed 0, until all of them \\ are exhausted. And one element is generated from each input Iterable DataPipes in turn, until \\ the end when the shortest input DataPipe is used up.\\ \\ \#\# Response\\ Please randomly select samples from these DataPipes using a random seed of 0. Keep selecting \\ samples until all of the DataPipes are exhausted. Additionally, generate one element from each \\ input Iterable DataPipe in a sequential manner, stopping when the shortest input DataPipe is used up.\\ \\ \#\# Query\\ Filtering by the above function Next, group the files by their file name using the group\_fn function. \\ Then, reserving the length of group result greater than 1.\\ \\ \#\# Response\\ Filter the files using the Next function, then group them by their file name using the \\ group\_fn function. Finally, keep only the groups with a length greater than 1.\\ \\ \#\# Query\\ Split into 2 sub-datapipes by the odd\_or\_even function Also split the source datapipe into two \\ datapipes by applying the function `great\_than\_5`\\ \\ \#\# Response\\ Can you please split the source datapipe into two datapipes by applying the function `great\_than\_5` \\ and also split it into 2 sub-datapipes using the odd\_or\_even function?\\ \\ \#\# Query\\ \{\{query\}\}\\ \\ \\ \#\# Response\end{tabular} \\ \hline
\end{tabular}%
}
\end{table*}
